Towards AI Logic for Social Reasoning

Artificial Intelligence (AI) logic formalizes the reasoning of intelligent agents. In this paper, we discuss how an argumentation-based AI logic could be used also to formalize important aspects of social reasoning. Besides reasoning about the knowledge and actions of individual agents, social AI logic can reason also about social dependencies among agents using the rights, obligations and permissions of the agents. We discuss four aspects of social AI logic. First, we discuss how rights represent relations between the obligations and permissions of intelligent agents. Second, we discuss how to argue about the right-to-know, a central issue in the recent discussion of privacy and ethics. Third, we discuss how a wide variety of conflicts among intelligent agents can be identified and (sometimes) resolved by comparing formal arguments. Importantly, to cover a wide range of arguments occurring in daily life, also fallacious arguments can be represented and reasoned about. Fourth, we discuss how to argue about the freedom to act for intelligent agents. Examples from social, legal and ethical reasoning highlight the challenges in developing social AI logic. The discussion of the four challenges leads to a research program for argumentation-based social AI logic, contributing towards the future development of AI logic.

==> 2_AIlogic_old.tex <==
\section{Rights and Permissions in AI logic}

%*************

%For the background section 2, which explains the various logics, I think we need to explain in particular the relation between rights and permissions on one hand, and prohibitions and obligations on the other hand. This has already been incorporated from what you wrote. There are two issues.

%1. The relation between the rights and permissions of an agent with his own prohibitions and obligations, I.e. the difference between weak and strong permissions

%2. The relation between the rights and permissions of an agent with the prohibitions and obligations of other agents, I.e. the difference between permissions and rights

%*************

AI logic formalizes the practical reasoning of intelligent autonomous agents. In this paper, we use an AI logic that has two distinctive features with respect to classical logic. In this section, we explain how  AI logic extends classical logic with modal operators for actions, beliefs, knowledge, right, obligations and permissions of intelligent autonomous agents. 
%Leon: I removed this as it is not explained what this means
%A deontic epistemic action logic for AI in social reasoning is presented here. 
In the following section, we explain how AI logic uses techniques from formal argumentation to represent common-sense reasoning, and deals with uncertainty, conflicts and exceptions. 
%These two aspects are explained in this introduction, and then used to formalize various aspects of social reasoning in the remainder of this paper.
We use the following running example in this section.

\begin{example}[Sensitive data scenario] \label{exam:data}
	%The first example is about sensitive data. 
	Someone's health data counts as sensitive data and as such is subject to strong protection principles in most of the countries (in the European Union to so-called GDPR, Regulation (EU) 2016/679 of the European Parliament and of the Council of 27 April 2016 on the protection of natural persons with regard to the processing of personal data and on the free movement of such data, and repealing Directive 95/46/EC). This means that others are not allowed to know these data. However, if someone is ill and in need of a treatment, we would all agree that the doctors have to provide this treatment. But fulfilling this obligation of them requires that they know the data of the agent's (in this case, patient's) health. 
\end{example}

Various claims from the example scenario above are visualized in Figure 1 below, together with a formalization in  AI logic. Moreover, the claims are grouped in two arguments visualized using vertical arrows.  The four claims on the left constitute the argument with conclusion that the doctor is not permitted to know the sensitive information, and the four claims to the right constitute the argument that the doctor is permitted to know that. The top claims are the conclusions of the argument, and the other claims are supporting those conclusions. Moreover, the fact that the doctor's permission to know prevails is modelled by the arrow from the top right box to the left top box. In this section we consider only the natural language statements and their formalization in  AI logic. The argumentation aspects are discussed in more detail in Section 3. 

\subfile{8_Examples_Graphs1}


\subsection{Language of modal AI logic}

Consider a classical logic language with formulas like {\it illness} and {\it treat}, to represent that the patient is ill and the patient has been treated. We can also add variables, such that {\it illness(patient)} represents that the patient is ill, and {\it treat(doctor, patient)} represents that the doctor is treating the patient. Moreover, considering agents like {\it doctor, patient} and {\it Suzy}, in  modal logic we can have formulas like $K_{\mbox{\it doctor}}$({\it illness}) to express that the doctor knows that the patient is ill, and $\neg K_{\mbox{\it patient}}$({\it illness}) to express that the patient does not know that he or she is ill. Here we may adopt the usual assumption in epistemic logic that beliefs may be mistaken but knowledge must be correct. In other words, when a doctor knows that the patient is ill, then this implies that the patient is ill. For example, knowledge may be modelled as justified, true belief. 



We consider social aspects like rights, obligations and permissions. For example, $O_{\mbox{\it doctor}}$({\it treat}) may express that for the doctor it is obliged that the patient is treated, and $P_{\mbox{\it patient}}$({\it illness}) may express that the patient is permitted to be ill. In some cases we can also index the modal operators with two agents in order to express that the obligation is directed (see Section 2.2), for example $O_{\mbox{\it doctor,patient}}$({\it treat}) may express that for the doctor it is obligatory with respect to the patient that the patient is treated, that is, this is a duty of the doctor toward the patient. In general, there are several ways in which an example can be formalized, and this is left to the person modelling the example.
%\subsection{Further developments in AI logic}
%Note for further development: BDI logic, causality, action and change, and so on. We can use the background literature for this.


Practical reasoning is about what agents do, so also actions must be represented in the language~\cite{horty2001agency}. For example [{\it doctor}] {\it treat} stands for the action that the doctor sees to it that the patient is treated. Finally, we use a universal modality $\Box$ to represent necessities, for example $\Box(illness\rightarrow sensitive)$ expresses that data regarding someone's health is sensitive data.


The advantage of modal logic is that all the expressions can be mixed in various ways, and this will be used extensively in this paper. For example $P_{\mbox{\it patient}}K_{\mbox{\it doctor}}$({\it illness}) represents that for the patient it is permitted that the doctor knows about the patient's illness. We can also represent universal permissions and obligations by leaving out the agents. An example is $P K_{\mbox{\it doctor}}$({\it illness}).

\subsection{Rights representing social dependencies} \label{sec:right}

Rights play a central role in this paper, since they point out a crucial social phenomenon: how the agents' social (in the specific context: normative) positions depend on each-other and each-other's positions. It is well known that talking about ``rights'' in itself is ambiguous. This ambiguity easily leads to a conceptual obscurity, thus, a hundred year ago, an American legal theorist differentiated between the possible meanings \cite{Hohfeld,MarkovichSL}. In the system of Hohfeld, which consists of four different right-relations, there are four different rights, each comes with a given type of duty on the other side: someone's right always means \textit{someone else's} duty, he calls these pairs, that is, \textit{normative positions}~\cite{sergot13_normative} at the ends of the four possible relations, correlatives, as they always come together (which, from a logical point of view, will be equivalence). The system Hohfeld drew can be graphically represented in the following way (rights in the upper row, duties are the lower one):

\begin{center}
\begin{tikzpicture}[scale=3, >=stealth, line width=.5mm]
% baloldali �bra
\begin{scope}[]
\node (v1) at (0,0) {duty};
\node (v2) at (0,1) {claim-right};
\node (v3) at (1,1) {freedom};
\node (v4) at (1,0) {no-claim};
\draw[<->]  (v1) -- (v2) node[midway, above, sloped]{\footnotesize correlatives};
\draw[<->]  (v3) -- (v4) node[midway, below, sloped, rotate=180]{\footnotesize correlatives};
\draw[<->, blue]  (v2) -- (v4);
\draw[<->, blue]  (v1) -- (v3);
\node at (0.5,0.75) {\footnotesize opposites};
\end{scope}
%jobboldali �bra
\begin{scope}[xshift=2cm]
\node (v1) at (0,0) {liability};
\node (v2) at (0,1) {power};
\node (v3) at (1,1) {immunity};
\node (v4) at (1,0) {disability};
\draw[<->]  (v1) -- (v2) node[midway, above, sloped]{\footnotesize correlatives};
\draw[<->]  (v3) -- (v4) node[midway, below, sloped, rotate=180]{\footnotesize correlatives};
\draw[<->, blue]  (v2) -- (v4);
\draw[<->, blue]  (v1) -- (v3);
\node at (0.5,0.75) {\footnotesize opposites};
\end{scope}
\end{tikzpicture}
\end{center}

These positions emerge most visibly in case of a contract: the seller's (claim-)right to the purchase-price obviously means the buyer's duty to give it to her. But this phenomenon is way more general. Regarding the epistemic positions, if someone has a (claim-)right to know something, it means that the other agent has a duty directed toward the previous one to tell him: $R_a[b]K_a\varphi \Leftrightarrow O_{b,a}[b]K_a\varphi$. If someone has a freedom to know something, though, that only means that the other agent has no (claim-)right toward him that he doesn't (get to) know. We usually consider this position really a freedom when no other agent has a (claim-)right that the agent shouldn't (get to) know that thing, which we usually refer to as \textit{permission}, which we will analyze in the next subsection.
%let's say that we have a piece of land. In the case, we have a freedom to walk through it $P_{we}(we-enter)$, which, in the Hohfeldian system means that the other agent we consider has no claim towards us not to do so $\neg R_{others}\neg(we-enter)$.
 % (that is, the notion of freedom is practically~\footnote{`Practically' as in the Hohfeldian system we consider the relation of two agents, not a general impersonal situation, but as we will see, we can move from one to the other.} the same what we told to be the weak permission: the absence of a prohibition). 
 %We, though, do have a claim-right toward the other agent to keep out $R_{we, others} \neg (other-enter)$: he has a duty (in the narrow sense) not to walk through on it $O_{other}\neg(other-enter)$. 
 The square on the right-hand side exhibit a very similar structure, those positions, though, are dynamic~\cite{kanger1966rights,lindahl1977position}, those are about the \textit{potential} to change other's rights and duties~\cite{MarkovichSL}. For example, if we mean the right to know something as a power, that means that the agent having this power can put a duty directed on the other agent---whose position is called liability in this system---to let her know: $Power_{a,b}[a]O_{b,a}[b]K_a\varphi$. Meanwhile, if someone has an immunity regarding her knowledge, we would mean that the other agent has no power to put a duty on her to tell him (about the details of formalizing power and the related positions see  \cite{dong2017dynamic,MarkovichSL}).
 %If we have this land, we have the power to sell it, this will change the related normative relations, our claim-rights will then disappear, the new owner will have them  ($P_{we}[we](\neg R_{we,others}\neg(other-enter) \wedge R_{new,other}(other-enter))$). Whoever can be affected by these changes are in a positions of the so-called Hohfeldian liability (which is not the same what we nowadays call legal liability). If we are the owners, others cannot sell it, what is more, they cannot tell us not to walk through on it: we have the immunity regarding this, which means, they are disable to put such a duty on us.
%Not just the types of rights (or at least some of them) resemble (more or less) to permission: the duty is a special type---or narrower interpretation---of obligation. 

\sout{As it can be seen, the original system of Hohfeld considered pairs of agents, but it can be generalized, and with taking the conjunction of the distinct relations of the same kind with regards all he other agents, we can gain the ``classical'' deontic notion: duty is a directed obligation, we talk about two agents' relation and their position, the obligation of an agent is directed toward to the other one (the classical example of which is the duties one undertakes in a contract: he has to fulfil them toward the other agent), but we have a duty to not kill \textit{any other agent}, that is, we have an obligation not to kill, we don't need to indicate toward whom this duty exist:} it's general $O_a\neg[a](kill)$, what is more, if we consider this obligation as being general in the sense of being valid for everyone, focusing only on the result that no one should be killed, we might say: $O\neg(kill)$.

The agency of the action and the normative position interact~\cite{sergot13_normative}, in the sense that we can have freedoms regarding  actions (this is a so-called active rights), while we can only have claim-rights regarding some other agent's action (passive rights). Power is active: it's about the potential that we can use with  action (e.g. by commanding something to the other agent), immunity is passive as it is about the missing potential of the other agent. We could think that it is already very decisive as form the rights' natural language phrase it will turn out whose action it concerns. Sometimes it is not clear though, from first reading, as we might see in the scope a notion incorporating different things, different atomic rights of the Hohfeldian types. The right to privacy (see in the example of sensitive data) covers many things, for example (claim-)rights towards everyone else to keep away from the private zone, that is, not to get to know about one's private life---which means a long list of prohibitions: any action which might end up gathering and disclosing information regarding the private zone (see the in Example~\ref{exam:data}).
%Hohfeld elaborated his system to describe legal rights, but it is important to emphasize that it draws a more general system: the theory can be applied to many kinds of systems existing outside of the world of law, like institutions, where it has to be clear who has what kind of duties toward whom and who can put a duty on whom (who has the power), or to go even further, to computer specifications~\cite{jones1996formal,grossi2008many}.
%{\bf Add some formulas from Example 1 to the following paragraph} \HM{I put some here. Maybe Reka would check and revise them?}
%In our AI logic we can also express the right to know. If someone has a right to know something, like ``The doctor is permitted to know about the patient's illness'' ($PK_{doctor}(illness)$), then it means that there is someone who has the duty to see to it that the aforementioned agent know that something, e.g. ``The doctor cannot treat a person if she doesn't know about the illness'' ($\Diamond\langle doctor \rangle(treat) \rightarrow K_{docter}(illness)$). Reka: no, here we talk about permisson (freedom), not right. 
%\HM{It seems that we need the Snowden case to clarify the notion of right to know, as argued below. }
These rights, like most of the rights (there are a very few exceptions in the modern constitutional democracies) are defeasible. This property means that their existence (the truth of the sentences expressing them or the inferences we would draw from them) might depend on circumstances. It might happen that the information that someone right to know would concern is secret for some reason and there are stronger arguments keeping it so and the ones supporting the agent's right to know it---in this case, there is no obligation to let them know (what is more, these latter arguments often support a prohibition regarding letting them know). Or the other way around: someone's right to privacy, which would mean that other shouldn't know about their private life and information, can also be defeasible: it can be the case that what they do in their private life might be dangerous for others, and public interest is often a strong argument against the individual one. Sometimes it is far from easy to decide which argument is stronger and then we face a dilemma. Both cases can be represented with using formal argumentation (see in Section~\ref{sec:another}).
% \HM{Could Reka illustrate the notions like \emph{reasons}, obligations, defeasibility in above? Reka: well, we have nothing in our language for reasons, so I don't know what illustration you would expect}
%\\\indent We present three examples, the reader can find their graphs at the end of the paper. The first example is about sensitive data. Someone's health data counts as sensitive data and as such is subject to strong protection principles in most of the countries (in the European Union to so-called GDPR, Regulation (EU) 2016/679 of the European Parliament and of the Council of 27 April 2016 on the protection of natural persons with regard to the processing of personal data and on the free movement of such data, and repealing Directive 95/46/EC). This means that others are not allowed to know these data. However, if someone is ill and in need of a treatment, we would all agree that the doctors have to provide this treatment. But fulfilling this obligation of them requires that they know the data of agent's (in this case, patient's) health. This first case seems to be easily decidable. 
%\\\indent The second example, though, presents an existing debate, the debate related to abortion. It is a widely shared thought that the expectant parents have a right to know whether the foetus is expected to be a healthy child after birth which means that the doctor has to tell them if this is the case. One argument supporting this is that they have a right to decide whether they want to have a baby which is expected to be seriously ill---and in order to decide, they need to know about it. This means that abortion is permitted. There is an other, actually contradicting opinion saying that the abortion is very wrong and what supports this is that everyone has a right to life, that is, all the others---also the expectant parents---are forbidden to take this life. This support (the relation between the two latter claim) can be attacked by saying that life as such starts with birth, that is, having an abortion doesn't violates anyone's right to life. In Texas, USA, the senate accepted a bill declaring that parents who had a seriously ill baby born, cannot sue the doctor because of not identifying this illness during the pregnancy. As it is argued in \cite{MarkovichSL} if something (or its compensation) is not subject to enforcement in court, then it is not subject of a duty. This means that in Texas, the expectant parents have no right to know whether their foetus is expected to be healthy or not, as the doctor don't have to tell them. 
%\\\indent The third example is also a well-known existing debate where the right to know and the prohibition to let others know collide. Edward Snowden worked for the CIA and, therefore knew about what surveillance the CIA conducted. Surveillance as such violates the right to privacy: during surveillance the conducting agent gathers private information about the other, who doesn't even know about this. We might agree in that peple have a right to know that their rights are violated, this dictates that Snowden, who knew that this was the case, had to tell them (and leaking the information was exactly he morally had to do). But from a labour law point of view, one as an employee might know information that others shouldn't, so he shouldn't tell them. Also, surveillance might have happened with good reason (as we mentioned above, the right to privacy is defeasible) and in this case leaking the information might have endangered the public interest. This means that Snowden shouldn't have done it.

\subsection{Free-choice permission} \label{sec:fcp}




%Given that as a doctor is permitted to treat the patient, if it were a weak permission, it is uncertain whether the doctor is permitted to know the patient's medical record without given that this is not forbidden. Yet, as a strong permission subject to medical norms, and as a knowledge that knowing the patient's medical record is necessary for the treatment, the doctor can check this sensitive information freely. 


%``If $a$ is weakly permitted, there is at least one way of doing it that does not lead to a violation. If it is strongly permitted, then no ways of doing it lead to a violation''~\cite{dignum1996free}.


% defeasible effect/exception of existing norms (``the other has a duty not to interfere''~\cite{raz1994ethics})




%\subsubsection{Weak Permission: Absence of Prohibition}
Handling the notion of permission in logic on a systematic level started at the same time as handling obligation: with creating the so-called deontic logic \cite{deonhandbook}, which we usually ascribe to Georg von Wright \cite{vonWright1951}.
Von Wright's sense of weak permission, usually, is understood as ``the lack of prohibition''. So the expression ``it is permitted'' is supposed to mean``it is not forbidden''. This reductive account simplifies weak permission as the negation of forbiddance, or, in other words, the dual of obligation. This interdefinability is one of two basic axioms in standard deontic logic~\cite{mcnamara2006deontic}. Therefore, weak permission adopts the \emph{upward} principle as the possibility modality does in normal modal logic: ``If it is  permitted to check the patient's medical record, then it is permitted to check the patient's sensitive data'' $P_{doctor}(record) \rightarrow P_{doctor}(sensitive)$, given that medical record is one kind of sensitive data $\Box(record \rightarrow snesitive)$.

Yet it is inevitable that the feature of closed \emph{upward} let weak permission have too strong derivation power than we need in social reasoning. Weak permission brings us back to a variant of Ross' paradox~ \cite{mcnamara2006deontic}. Given that it is permitted to check the patient's medication record, it then infers that it is permitted to check the patient's medication record or sell it to the insurance company $P_{doctor}(record) \rightarrow P_{doctor}(record \vee sell)$~\footnote{Since, as we mentioned above, a permission always concerns the agent's action whose permission we talk about $P_{doctor}(record)$ or $P[d](record)$ are shorter versions of writing that $P_{doctor}[doctor](record)$.}. But the latter is not ethically or legally allowed to do. 



%\subsubsection{Strong Permission: Freedom to Act}

Von Wright later said, ``(Strong) [p]ermission (...) means freedom to choose between all the alternatives, if any, covered by the permitted thing''~\cite[p.32]{von1968essay}. This ``open'' flavor of ``freedome to chose'' is well known in philosophy as permission \emph{at liberty}~\cite{raz1975permissions}, and also commonly occurs in term of ``discretion'' in ordinary language and legal context: 
\begin{itemize}
	\item ``Exactly how much to tip a server is at the discretion of the customer.'' %(Merriam-Webster)
	\item ``Bail is granted at the discretion of the court. ''
%	\item ``Whether or not you get a bonus is at your boss's discretion, so you better impress her!''
\end{itemize}
In contrast to weak permission, the open sense is \emph{downward} closed but restricted: ``If it is permitted to know the patient's sensitive information, then it is permitted to know the patient's medical record'' $PK_{doctor}(sensitive) \rightarrow PK_{doctor}(record)$, as the knowledge of that medical record is a type of sensitive data $\Box(record \rightarrow sensitive)$. This kind of permission has been developed by van Benthem in modal logic~\cite{van1979minimal}, in which strong permission not only has to follow the axiom in this open sense, but also have to obey the axiom called ``obligation as the weakest permission''~\cite{ano2015symbolic}. The latter gives the ``non-violation of norm'' restriction for strong permission: All strong permissions have to stay inside the zone set up by obligations. While the doctor may know and use the patinet's e-mail address to communicate with him, it is forbidden to misuse the patient's data, for example, she cannot send spam to him $O_{doctor}\neg(spam)$. This prohibition and the permission for the doctor to know and use the patient's e-mail address $PK_{doctor}(email)$, the doctor knows that (normally) what is permitted is restricted by the prohibition $K_{doctor}(email \rightarrow \neg (spam))$. This is similar to von Wright's viewpoint shown beforehead~\cite{vonWright1963}.  

Some may argue that the derivation power of strong permission is still too strong and thus faces some difficulty in social reasoning, given the free choice permission paradox~\cite{hansson13:_variet_permis}. The worry concerns that \emph{downward} closure can be led given some non-normal knowledge: Permitting the doctor to check the patient medical record, then the doctor is permitted to know the record and destroy it $PK_{doctor}(record) \rightarrow P(K_{doctor}(record) \wedge destroy)$, if it is the case that the doctor's knowing the record and destroying it (normally) is a case for the doctor to know the record $\Box(K_{doctor}(record) \wedge destroy \rightarrow K_{doctor}(record))$. Yet this condition does not look like a (normal) knowledge in daily life. We will give a further analysis of strong permission in Section~\ref{sec:fcp}.

Since  claim-rights are often declared in legal or moral codes, they might be mixed up with the what we called strong permission~\cite{von1968essay}. However, a permission, weak or strong, always concerns our own action, not someone else's. Permission exhibits stronger resemblance to power. In some sense, both refer to some normative possibility of ours. There is a very important difference though in their consequences, as Makinson points out in \cite{Makinson}: if we do something without permission, the consequence will be some punishment. However, if we try to do something without power, we won't be able to do it: as it is argued for in \cite{MarkovichSL}, power concerns actions which are created by constitutive rules (the theory of which is well-known in the presentation of Searle \cite{Searle}). We cannot sell something if it is not ours: selling is a constituted notion (action), the rules describing what happens when someone sells something constitute it. Property on a thing involves a power to sell, if we don't have it, we cannot sell the thing.
%The open sense of permission is more natural when agencies do not have complete knowledge of the world~\cite{dignum1996free}. 



% Huimin's points:

%1* When I bid for strong permission, I am not saying that I would bid the intuition of “freedom to act” than “act without prohibition”. What I would say here is more likely to compare the reasoning powers of these two permissions, and goes for strong permission as it can offer us more derivation results than weak permission does. In addition, strong permission sounds to be more possible to guide my actions than the other does. This may fit with the linguists’ viewpoint like Leon mentioned. 

%2* I would say that strong permission can capture both intuitions, “freedom to act” and “act without prohibition”, which cannot be done by weak permission. Furthermore, the legal term “all is permissible unless prohibited” can be fully captured by strong permission as the idea of freedom it offers, while this cannot be done in weak permission. I will argue this in two ways, by comparing their intuitions and by comparing their reasoning powers. 

%3* Intuitively speaking, I would consider weak permission as offering "one possible way to act", a way without being prohibited; but we don't know what is the exact way to act without prohibition. While, strong permission to me sounds like the "freedom to do", going for "all possible ways to act" if no exceptional act occurs. In this sense, it sounds to me that strong permission offers a sense of action guiding: all expected acts regarding to this permission are allowed.

%4* I agree that the formal definition of weak permission is a simple way to model “absence of prohibition”, but in the viewpoint of logical reasoning, or linguistic viewpoint, it cannot offer enough derivation power as this legal term means. Weak permission only says that there is such a way, but we don’t know which. It is more likely to say “We are allowed do this, but sorry that I cannot tell in which specific way really works without prohibition”. The reason is that, mathematically speaking, the concepts of weak permission are closed upward. 

%5* Given that I am permitted to drink beer and smoke after 16, weak permission says that I am permitted to drink beer and I am permitted to smoke. Because this weak permission only states a possibility to do both actions together. This leads to that they both are also possible. So far so good. But knowing that I am permitted to drink beer after 16, if we check more clear, weak permission does not tell me clearly whether this possibility is to drink beer in a bar or is to drink beer at home. I only know that I am permitted to drink beer in a bar, when there is a piece of ADDITIONAL information saying that drinking in a bar after 16 is not prohibited. In conclusion, to derive more specific weak permission, we need additional information. 

%6* First strong permission is able to capture the idea of “absence of prohibition”. Intuitively speaking, strong permission offers a freedom to act in whatever way you want, but staying inside the zone set up by laws. To me this is the meaning of having a license. 

%7* Also, strong permission is more closer to the concept of “all is permissible unless prohibited” than weak permission does, as the format of “ALL” it states. Suppose I get the key of the office from University of Luxembourg, and thus this license giving me the right to use the facilities regarding to the office. This right, seems to me, let me understand all expected ways to stay at the building, have a desk under my name (temporally), and use the coffee machine when I want. 

%8* You may say that weak permission also works in the right to use situation. But as argued before, to understand the more specific situation from weak permission, we need more information. In contrast, strong permission automatically gives us all expected and permissible actions. In other words, strong permission needs less information to give us more possible results.   

%9* This difference can be captured by using argumentation theory. Given a knowledge base with statements “It is permitted to drink beer after 16”, “Ought not to drink and drive”, and “drink and drive is a possible way to act”. If we think about weak permission, we cannot infer that “It is permitted to drink beer in a bar after 16”. For strong permission, we can say something more: “It is permitted to drink beer in a bar after 16” and “It is not permitted to drink and drink”. 

\subsection{Permission to Know in Social Reasoning}


Consider knowledge with normative notions in social and moral reasoning, one interesting concept this interaction bringing about is permission to know. As argued in Section~\ref{sec:right}, one has a right to know implies the other own their duties to see to it happens. This can be extended into other aspects in social reasoning. As a citizen you are allowed to know the documentories of the city. You make a data inquiry and then the archives should send you back the data you enquired. So the form of $P_a[b]K_a\varphi \rightarrow O_{b,a}[b]K_a\varphi$ holds in this scenario. However, if we still think knowledge involved here should be classical as ``justified true belief'', namely knowledge implies truth, then we will get to a weird conclusion $O_{b,a}[b]\varphi$ from the premise of permission to know $P_a[b]K_a\varphi$. It is not clear whether knowledge still implies truth, interacting with normative notions. Similar challenges of knowledge occur in the other aspects of social reasoning~\cite{fagin2004reasoning}. One famous case is called the Moore paradox~\cite{van2007dynamic}, which engages the ``pragmatically paradoxical formula'' $K_a(\varphi \wedge \neg K_a\varphi)$. In which sense of knowledge we want to have, when we are modelling our natural language of permission to know? This is an important issue in social reasoning. 


%is responsibility~\cite{sep-moral-responsibility}. Given the doctor knows the situation of the patient $K_{doctor}(illness)$, he should treat the ill person $O_{doctor}\langle doctor \rangle (treat)$; otherwise the doctor will be sued for failling his duty. 

%Example: Responsibility without and within knowledge. 

%Social dependency for Coordinated Attack



%Despite  ``justified true belief'', knowledge has many faces in epistemic reasoning~\cite{fagin2004reasoning}, meanwhile representing different forms of social dependency, like the notions of ``everyone knows'', ``wise man knows'', and common konwledge. They have been widely discussed in artificial interlligence as well~\cite{mccarthy1978model}. 


%awareness~\cite{hans,emiliano}, memories~\cite{ram}, lies~\cite{Hans,Thomas}, information pooling~\cite{Yiresolve,Olivier}



%----Reka----
%I haven’t figured it out how the right to know should be. What is sure, it is not RK(p v ~p) because of two reasons: you wrote one, the other is that it wouldn’t make sense to say something like this in terms of rights: the parents know already that the foetus is either healthy or not, what they have the right to know is which one, and the closest solution is the conditional we (I guess Leon) wrote on the white board. So I’m working on that, the 10 points is only the “background”.




%-----Reka------
%This doesn't concern this paper directly, just came to my mind as I read that "Mary doesn't know that the window is open" that while in S5 from this sentence it doesn't follow that the window is open, pragmatically it does. We don't say that someone doesn't know something unless that something is true. For the sentence "Réka doesn't know that the Earth is flat" most people would say that something is wrong with the sentence, they wouldn't say it's true. Wrong in the sense like famous "The present king of France is bald", however here the other option is the false (not the true): this latter presupposes that the there is a king of France, which there isn't, so, according to Russell, we cannot assign truth value to this sentence. The "Réka doesn't know that the Earth is flat" feels to presuppose that the Earth is flat, which it isn't, but this presupposition would mean implication in the logical sense, which is not the case in S5. 

%I know that we don't want to write about this, I just wanted to write it out loud in order to not forget to check later how this has been discussed (because I'm sure it has been, my knowledge is pretty superficial regarding epistemic logic).





%-----Leon------
%It is also related to the notorious Moore sentences underlying DEL: informing”the earth is flat and Reka does not know it” make the information false (because now Reka knows that the earth is flat). So in the mechanism, “Reka does not know that the earth is flat” comes with the factual expression.

%One problem with language is that the line between semantics and pragmatics is a bit fuzzy. As a first indication, one may say that all nonmonotonic consequences are pragmatics. (Though Cleo explained me this was a bit too simple)

%So we can suggest, for example, that the inference of the permission for knifed murder from the permission to use a knife is just a pragmatic inference. Likewise, we can suggest that the inference of a from PKq is just pragmatics. The problem is that we are not linguists so it may mean something else than we would like it to mean.


\subsection{Conflicts among agents in AI logic}

%{\bf Before introducing argumentatton theory, explain the general idea of non-monotonic logic. Refer to volume 3 of the handbook of logic in AI and LP~\cite{gabbay1994handbook}, which addresses this in some detail. Also add reference to the Nute book on defeasible deotnic logic~\cite{nute2012defeasible}, and Leon's PhD thesis~\cite{torre97}. And Goble's chapter in the handbook of deontic logic, volume 1~\cite{goble2013prima}. Gabby on non-monotonic reasoning~\cite{gabbay1985theoretical}} \HM{Done. Please check this section. }

%Formal argumentation is around 
{\bf Cite BOID here for conlicts among agents, and how to resolve some of these conflicts}

The beliefs of two agents may be different, and then we can see that the agents conflict. However, there are much more ways in which two agents can be called conflicting. For example, they may try to execute actions with contradictory consequences. Or they may have incompatible rights.

In the following section we introduce formal argumentation among agents to represent conflicts between logical formulas. There are two ways to define conflicts in logic. First we can use a formal semantics, and then there is a conflict if there is no model of the sentences. The semantics of modal logic is based on possible worlds. So for each modal operator there is a set of accessible worlds, and a formula like $O\phi$ is true when $\phi$ is true in all accessible worlds. If the semantics is based on accessible worlds with serial relation, we cannot have a model together for sentences like $O\neg(treat)$ and $O(treat)$. Otherwise the model would be empty. Alternatively, we can define a proof system for  modal logic, and then there is a conflict given a set of premises if we can derive a formula and its negation. An additional advantage of a proof system is that the axioms of the proof system reflect the characteristic properties of the logic. For instance, van Benthem's logic~\cite{van1979minimal} has two axioms to characterize permission and obligation (see in Section~\ref{sec:fcp}). 

Reasoning in social reality is not deductively valid like in modal logics, but rather it is uncertain and wants conflict be resolved. Social reasoning with uncertainty is ubiquitous. The doctor is obliged to treat the patient given the patient is deadly ill ($ill \rightarrow O_{doctor}(treat)$). But the doctor is obliged not to do so if she does not know the patient's medical record ($\neg O_{doctor}\neg(treat) \rightarrow K_{doctor}(ill)$). So far so good. But when the scenario is that the patient is ill but the privacy of the patient stops the doctor to know the patient's medical record, namely the set of assumptions is $\{ill, \neg K_{doctor}(ill)\}$, then we conclude with $O_{doctor}(treat)$ and $O_{doctor}\neg(treat)$, the doctor's obligation to treat the patient and her obligation not to treat the patient. Which conclusion we should draw? This uncertainty reflects a normative conflict~\cite{ginsberg1994ai,goble2013prima} AI logic wants to resolve~\cite{torre97,nute2012defeasible}. 

As argued in~\cite{gabbay1985theoretical,gabbay1994handbook,nute2012defeasible}, a key property of intelligence is to deal with the \emph{uncertainty} of the conclusions we draw in social reasoning, when a new piece of evidence as \emph{exception} is given. The general idea of handling this issue in non-monotonic reasoning, as we already mentioned above, is called ``\emph{defeasibility}''. 

{\bf This section is a bit unsatisfactory since it uses manyunexplained terms, such as defeasibility. also defeasibility is explained only in section 3, when we talk about argumentation. There is no defeasibility in the AI logic discussed in this section thus far.}\RC{I talk about defeasibility of rights, I intentionally did it in a very introductory way preparing the question to be discussed later (more) formally in the paper. It's not ok this way?} \HM{Yes, please do this Reka.}

% ``intimately conected with defeasible nature of commonsense inference [$\dots$]; we are all capable of drawing conclusions, acting on them, and then retracting them if necessary in the face of new evidence''~\cite{ginsberg1994ai}.

%\subsection{Old text}

%{\bf This part used to be in the section on rights but since we discuss rights first, now we need to discuss the relation in the permission section: (that is, the notion of freedom is practically~\footnote{`Practically' as in the Hohfeldian system we consider the relation of two agents, not a general impersonal situation, but as we will see, we can move from one to the other.} the same what we told to be the weak permission: the absence of a prohibition). }


%{\bf Same: 
%As argued in~\cite{hohfeld1913some,hansson13:_variet_permis}, it is far from obvious what properties the so-called permission should have. There are some further notions which show strong resemblance to permission, especially in their natural language appearance, but have very different consequences: these are the so-called rights~\cite{hohfeld1913some}, of which we can distinguish at least four different types~\cite{sergot13_normative}. Since their natural language appearance is the source of our knowledge regarding them, differentiating them and using the proper one in the formalization for AI logics is an essential task.}



==> 3_Static_Dynamic_Rights.tex <==

\section{Rights and Duties}
As we have seen, it is far from obvious what properties the so-called permission should have. There are some further notions which show strong resemblance to permission, especially in their natural language appearance, but have very different consequences: these are the so-called rights, of which we can distinguish at least four different types. Since their natural language appearance is the source of our knowledge regarding them, differentiating them and using the proper one in the formalization for AI logics is an essential task.
\\\indent Talking about `rights' in itself is ambiguous. This ambiguity easily leads to a conceptual obscurity, thus, a hundred year ago, an American legal theorist differentiated between the possible meanings \cite{Hohfeld}. In the system of Hohfeld there are four different rights, each comes with a given type of duty on the other side: someone's right always means \textit{someone else's} duty, he calls these pairs, that is, \textit{normative positions} at the ends of the four possible relations, correlatives, as they always come together (which, from a logical point of view, will be equivalence). The system Hohfeld drew can be graphically represented in the following way (rights in the upper row, duties are the lower one):
\\
\begin{tikzpicture}[scale=3, >=stealth, line width=.5mm]
% baloldali ábra
\begin{scope}[]
\node (v1) at (0,0) {duty};
\node (v2) at (0,1) {claim-right};
\node (v3) at (1,1) {freedom};
\node (v4) at (1,0) {no-claim};
\draw[<->]  (v1) -- (v2) node[midway, above, sloped]{\footnotesize correlatives};
\draw[<->]  (v3) -- (v4) node[midway, below, sloped, rotate=180]{\footnotesize correlatives};
\draw[<->, blue]  (v2) -- (v4);
\draw[<->, blue]  (v1) -- (v3);
\node at (0.5,0.75) {\footnotesize opposites};
\end{scope}
%jobboldali ábra
\begin{scope}[xshift=2cm]
\node (v1) at (0,0) {liability};
\node (v2) at (0,1) {power};
\node (v3) at (1,1) {immunity};
\node (v4) at (1,0) {disability};
\draw[<->]  (v1) -- (v2) node[midway, above, sloped]{\footnotesize correlatives};
\draw[<->]  (v3) -- (v4) node[midway, below, sloped, rotate=180]{\footnotesize correlatives};
\draw[<->, blue]  (v2) -- (v4);
\draw[<->, blue]  (v1) -- (v3);
\node at (0.5,0.75) {\footnotesize opposites};
\end{scope}
\end{tikzpicture}

These positions emerge most visibly in the case of a contract: the seller's right to the purchase-price obviuosly means the buyer's duty to give it to her. But this phenomenon is way more general: let's say that we have a piece of land. In the case, we have a freedom to walk through it, which, in the Hohfeldian system means that the other agent we consider has no claim towards us not to do so (that is, the notion of freedom is practically\footnote{`Practically' as in the Hohfeldian system we consider the relation of two agents, not a general impersonal situation, but as we will see, we can move from one to the other.} the same what we told to be the weak permission: the absence of a prohibition). We, though, do have a claim-right toward the other agent to keep out: he has a duty (in the narrow sense) not to walk through on it. The square on the right-hand side exhibit a very similar structure. If we have this land, we have the power to sell it, this will change the related normative relations, our claim-rights will then disappear, the new owner will have them. Whoever can be affected by these changes are in a positions of the so-called Hohfeldian liability (which is not the same what we nowdays call legal liability). If we are the owners, others cannot sell it, what is more, they cannot tell us not to walk through on it: we have the immunity regarding this, which means, they are disable to put such a duty on us. 
\\\indent What we already have mentioned in these deontic notions is not the agents have a special interaction with the modalities: one's duty automatically means another one's right. It is also worth noting how the agency of the action and the normative position interact: we can have freedoms regarding our actions (this is a so-called active rights), while we can only have claim-rights regarding some other agent's action (passive rights). Power is active, immunity is passive. We could think that it is already very decisive as form the rights' natural language phrase it will turn out whose action it concerns. Sometimes it is not clear though, from first reading, as we might see in the scope a notion incorporating different things, different atomic rights of the Hohfeldian types. The right to privacy (see in the privacy example) covers claim-rights towards everyone else to keep away from our private zone, that is, not to get to know about our private life---which means a long list of prohibitions: any action which might end up gathering and disclosing information regarding our private zone (see the in example). 
\\
\\Since our claim-rights are often declared in legal or moral codes, they might be mixed up with the what we called strong permission. However, a permission, weak or strong, always concerns our own action, not someone else's. Permission exhibits stronger resemblance to power. In some sense, both refer to some normative possibility of ours. There is a very important difference though in their consequences, as Makinson points out in \cite{Makinson}: if we do something without permission, the consequence will be some punishment. However, if we try to do something without power, we won't be able to do it: as it is argued for in \cite{MarkovichSL}, power concerns actions which are created by constitutive rules (the theory of which is well-known in the presentation of Searle \cite{Searle}). We cannot sell something if it is not ours: selling is a constituted notion (action) the rules describing what happens when someone sells something constitute it. Property on a thing involves a power to sell, if we don't have it, we cannot sell the thing.
\\
\\Hohfeld elaborated his system to describe legal rights, but it is important to emphasize that it draws a more general system: the theory can be applied to many kinds of systems existing outside of the world of law, like institutions, where it has to be clear who has what kind of duties toward whom and who can put a duty on whom (who has the power), or to go even further, to computer specifications \cite{}
\\Not just the types of rights (or at least some of them) resemble (more or less) to permission: the duty is a special type---or narrower interpretation---of obligation. The Hohfeldian duty (in the narrow sense) only differs from the "classical" obligation in being directed: as in this system we always talk about two agents' relation and their position, the obligation of an agent is directed toward to the other one the classical example of which is the duties one undertakes in a contract: he has to fulfil them toward the other agent. But this system can be generalized: if we have a give duty toward everyone else (which means the conjunction of the duties) then we get back the undirected type of obligation about which deontic logic usually talks (see in detail \cite{MarkovichSL, Markovich}.
\\
\\%What does it mean in the terms of right to know? If someone has a right to know something then it means that there is someone who has the duty to see to it that the aforementioned agent know that something. These rights, like most of the rights (there are a very few exceptions in the modern constitutional democracies) are defeasible. It might happen that the information regarding the knowledge of someone else 


%Example hospital

%1. Does a patient have the right to know if he or she has a disease? How about the family members of the patents? 
%2. Does this right to know depend on the other things the patient already know? He or she can only know the disease if he or she can understand what it means? 
%3. What are the obligations that can be derived from such a right? Are these obligations defeasible (see the first item above in this email), Where does argumentation come in?

%4. What are the powers in this hospital setting?
%--- 
%Example goods, or university setting, or something else
%1. We are permitted to know ingredient of food we buy for allergies, you are forbidden to know the recipe, how to resolve the conflict in a concrete case

%2. You are only permitted to know the ingredients if you know got some training

%3. Your right to know, imposes the obligation for the shop owner or manufacturer to tell you

%4. You can obtain the right to know by ...


%Final though, maybe we can also add some insights from normative positions (in the sense of the handbook), the audience does not know this either


==> 4_Defeasible_Permission.tex <==


\section{Permission in Social Reasoning}




\subsection{Defeasible Permissions in ASPIC$^+$}

From the viewpoint of linguistics, the social reasoning of multi-agent interactioin has to balance the derivation power and the intuition behind normative concept: to derive the necessary deductive results, unless some \emph{exceptional} cases occur. In the previous cases, the derived results of non-ideal permission (weak or strong) are the exceptions and then should be defeated. Including additional norms of ``Ought not to check the patient's medical record or sell it to the insurance company'' and ``Ought not to use the patient's medical record and destroy it'' into the knowledge base, the non-ideal permissions can be defeated in the ASPIC$^+$ we developed in the previous section. 

A more concrete case of defeasible permission can be found in legal reasoning. It is about sensitive data (See more details in Figure~\ref{fig:doctor}). Someone's health data counts as sensitive data ($A_3$) and as such is subject to strong protection principles in most of the countries (in the European Union to so-called GDPR, Regulation (EU) 2016/679 of the European Parliament and of the Council of 27 April 2016 on the protection of natural persons with regard to the processing of personal data and on the free movement of such data, and repealing Directive 95/46/EC) ($A_1$). This means that others are not allowed to know these data ($A_2$). The prohibition of some others to know these data ($A_4$) thus exits. However, if someone is ill and in need of a treatment, we would all agree that the doctors have to provide this treatment ($B_1$). But fulfilling this obligation of them ($B_2$) requires that they know the data of agent's (in this case, patient's) health ($B_3$). In this case, the previous argument $A_4$ of prohibiting the doctor to know about the patient's illness becomes an exception. This exception, as shown in Figure~\ref{fig:doctor}, defeated by the doctor being permitted to know the illness ($B_3$), has shown the defeasibility of the principles of data protection. 


% Huimin's points:

%1* When I bid for strong permission, I am not saying that I would bid the intuition of “freedom to act” than “act without prohibition”. What I would say here is more likely to compare the reasoning powers of these two permissions, and goes for strong permission as it can offer us more derivation results than weak permission does. In addition, strong permission sounds to be more possible to guide my actions than the other does. This may fit with the linguists’ viewpoint like Leon mentioned. 

%2* I would say that strong permission can capture both intuitions, “freedom to act” and “act without prohibition”, which cannot be done by weak permission. Furthermore, the legal term “all is permissible unless prohibited” can be fully captured by strong permission as the idea of freedom it offers, while this cannot be done in weak permission. I will argue this in two ways, by comparing their intuitions and by comparing their reasoning powers. 

%3* Intuitively speaking, I would consider weak permission as offering "one possible way to act", a way without being prohibited; but we don't know what is the exact way to act without prohibition. While, strong permission to me sounds like the "freedom to do", going for "all possible ways to act" if no exceptional act occurs. In this sense, it sounds to me that strong permission offers a sense of action guiding: all expected acts regarding to this permission are allowed.

%4* I agree that the formal definition of weak permission is a simple way to model “absence of prohibition”, but in the viewpoint of logical reasoning, or linguistic viewpoint, it cannot offer enough derivation power as this legal term means. Weak permission only says that there is such a way, but we don’t know which. It is more likely to say “We are allowed do this, but sorry that I cannot tell in which specific way really works without prohibition”. The reason is that, mathematically speaking, the concepts of weak permission are closed upward. 

%5* Given that I am permitted to drink beer and smoke after 16, weak permission says that I am permitted to drink beer and I am permitted to smoke. Because this weak permission only states a possibility to do both actions together. This leads to that they both are also possible. So far so good. But knowing that I am permitted to drink beer after 16, if we check more clear, weak permission does not tell me clearly whether this possibility is to drink beer in a bar or is to drink beer at home. I only know that I am permitted to drink beer in a bar, when there is a piece of ADDITIONAL information saying that drinking in a bar after 16 is not prohibited. In conclusion, to derive more specific weak permission, we need additional information. 

%6* First strong permission is able to capture the idea of “absence of prohibition”. Intuitively speaking, strong permission offers a freedom to act in whatever way you want, but staying inside the zone set up by laws. To me this is the meaning of having a license. 

%7* Also, strong permission is more closer to the concept of “all is permissible unless prohibited” than weak permission does, as the format of “ALL” it states. Suppose I get the key of the office from University of Luxembourg, and thus this license giving me the right to use the facilities regarding to the office. This right, seems to me, let me understand all expected ways to stay at the building, have a desk under my name (temporally), and use the coffee machine when I want. 

%8* You may say that weak permission also works in the right to use situation. But as argued before, to understand the more specific situation from weak permission, we need more information. In contrast, strong permission automatically gives us all expected and permissible actions. In other words, strong permission needs less information to give us more possible results.   

%9* This difference can be captured by using argumentation theory. Given a knowledge base with statements “It is permitted to drink beer after 16”, “Ought not to drink and drive”, and “drink and drive is a possible way to act”. If we think about weak permission, we cannot infer that “It is permitted to drink beer in a bar after 16”. For strong permission, we can say something more: “It is permitted to drink beer in a bar after 16” and “It is not permitted to drink and drink”. 




==> 8_Examples_Graphs3.tex <==


%%%%%%%%%%%%%%%%%%

%\begin{figure}
%	\noindent
%	\makebox[\textwidth]{
%		\begin{tikzpicture}[scale = .8]
		
		
		% group 1
		
%		\node[mystyle1] (A) at (-5,5) {\scriptsize * People have a right to know whether their rights are violated. \\ $A_1 = \bigwedge_{a \in Agt} (R_a\varphi \land \neg \varphi) \rightarrow R_aK_a\neg\varphi $};
		
%		\node[mystyle1] (B) at (-5,1) {\scriptsize Whoever knows about it has to tell them. \\ $A_2 = A_1 \mapsto \bigwedge_{b \in Agt} (K_b\neg\varphi \rightarrow O_{b\rightarrow a}[b]K_a\neg \varphi)  $};
		

%		\node[mystyle] (C) at (4.5,1) {\scriptsize Snowden knows about what surveillance the CIA conducts.\\ $A_3 = B_2, B_3, C_4 \Mapsto K_s(surveillance)$};
		
%		\node[mystyle1] (D) at (-2,-2.5) {\scriptsize Snowden has to tell them.\\ $A_4 = A_2, A_3, C_5 \Mapsto \bigwedge_{b \in Agt} O_s [s]  K_b(surveillance)$};

		% group 2		

%		\node[mystyle] (A') at (1,8) {\scriptsize * Snowden works for the CIA. \\ $B_1 = s \in {CIA}$};

%		\node[mystyle] (B') at (1,5) {\scriptsize Snowden is allowed to know classified information. \\ $B_2 = B_1 \mapsto PK_s(classified)$};

%		\node[mystyle] (C') at (8,5) {\scriptsize * Data regarding surveillance is classified. \\ $B_3 = \Box(surveillance \rightarrow classified)$};

%		\node[mystyle3] (D') at (15,5) {\scriptsize * Others are not allowed to know classified information. \\ $B_4 = \bigwedge_{a \not\in CIA} \neg PK_a(classified)$};

%		\node[mystyle3] (E') at (12,1) {\scriptsize People are not allowed to know about the surveillance. \\ $B_5 = B_3, B_4 \Mapsto \bigwedge_{a \not\in CIA} \neg PK_a(surveillance)$};

%		\node[mystyle3] (F') at (12,-2.5) {\scriptsize Snowden is forbidden to tell them. \\ $B_6 = B_5 \Mapsto \bigwedge_{a \in Agt}  O_s \neg [ s]  K_a(surveillance)$};

% group 3

%		\node[mystyle] (A'') at (12,10) {\scriptsize * Everyone has a right to privacy.\\ $C_1 = \bigwedge_{b \in Agt} R_b(privacy_b)$};

%		\node[mystyle] (B'') at (12,14) {\scriptsize Others are not allowed to know what one does in her private life.\\ $C_2 = C_1 \mapsto \bigwedge_{a \in Agt/\{b\}} \neg K_a(private_b)$};

%		\node[mystyle1] (C'') at (4.5,16) {\scriptsize * Surveillance results in knowing what people know in their private life. \\ $C_3 = \Box ([ a ](surveillance) \rightarrow \bigvee_{b \in Agt/\{a\}} K_a K_b(private_b)$};

%		\node[mystyle] (D'') at (4.5,12) {\scriptsize * The CIA conducted several surveillances. \\ $C_4 = [CIA] (surveillance)$};

%		\node[mystyle3] (E'') at (-3,14) {\scriptsize The CIA violated people's right to privacy.\\$C_5 = C_2, C_3, C_4 \mapsto [ CIA ] \neg\ (privacy_b) $};

% dashed link: below left

%    \draw (A) -- (B) node[draw=none,fill=none,font=\scriptsize,midway,right] {Hohfeld};

%    \draw[dashed] (B) -- (-5, -1) -- (4.5, -1)node[draw=none,fill=none,font=\scriptsize,midway,above] {Modus Ponens} -- (C) ;

%    \draw[dashed] (D) -- (-2, 13.2);

% dashed links: below middle

%    \draw (A') -- (B') node[draw=none,fill=none,font=\scriptsize,midway,right] {Member};

%    \draw[dashed] (B') -- (1, 3) -- (8, 3) -- (C') node[draw=none,fill=none,font=\scriptsize,midway,left] {FCP + $PK_a \varphi \rightarrow P\varphi$};

%    \draw[dashed] (D'') -- (C);

% dashed links: below right

%    \draw[dashed] (9, 4) -- (9, 3) -- (15, 3) -- (D') node[draw=none,fill=none,font=\scriptsize,midway,left] {FCP };

%    \draw[dashed] (12, 3) -- (E');

%    \draw[dashed] (E') -- (F') node[draw=none,fill=none,font=\scriptsize,midway,right] {$\neg PK_b\varphi \rightarrow O_b\neg  [b] K_b\varphi$};


% dashed links: above

%    \draw (C'') -- (1.5, 16) -- (1.5, 12) -- (D'');

%   \draw (B'') -- (E'') node[draw=none,fill=none,font=\scriptsize,midway,above] {$(K_a\varphi \rightarrow \varphi)$ + $([a](\varphi \rightarrow \psi) \wedge [a]\varphi \rightarrow [a]\psi) $};


% defeats

%\draw[postaction={draw,line width=1.5pt,solid}, <->] (D) -- (F');
		
%		\end{tikzpicture}
%	}
%	\caption{Modelling the surveillance case. } \label{fig:surveillance}
	
%\end{figure}



